Language Agents for Detecting Implicit Stereotypes in Text-to-image Models at Scale

The recent surge in the research of diffusion models has accelerated the adoption of text-to-image models in various Artificial Intelligence Generated Content (AIGC) commercial products. While these exceptional AIGC products are gaining increasing recognition and sparking enthusiasm among consumers, the questions regarding whether, when, and how these models might unintentionally reinforce existing societal stereotypes remain largely unaddressed. Motivated by recent advancements in language agents, here we introduce a novel agent architecture tailored for stereotype detection in text-to-image models. This versatile agent architecture is capable of accommodating free-form detection tasks and can autonomously invoke various tools to facilitate the entire process, from generating corresponding instructions and images, to detecting stereotypes. We build the stereotype-relevant benchmark based on multiple open-text datasets, and apply this architecture to commercial products and popular open source text-to-image models. We find that these models often display serious stereotypes when it comes to certain prompts about personal characteristics, social cultural context and crime-related aspects. In summary, these empirical findings underscore the pervasive existence of stereotypes across social dimensions, including gender, race, and religion, which not only validate the effectiveness of our proposed approach, but also emphasize the critical necessity of addressing potential ethical risks in the burgeoning realm of AIGC. As AIGC continues its rapid expansion trajectory, with new models and plugins emerging daily in staggering numbers, the challenge lies in the timely detection and mitigation of potential biases within these models.

==> sections/problem_definition.tex <==
\begin{myDef}[\textbf{Text to Image}]
Text to Image is the process of generating an image from a natural language textual description. We can represent the Text-to-Image model $G$ as a function that takes a natural language textual description (prompt) $\mathbf{z}$ as input and generates an image $\mathbf{x}$ as output. This function can be represented as:
\begin{equation}
    \mathbf{x} = G(\mathbf{z}).
\end{equation}
\end{myDef}

These generative models generate images based on textual descriptions, which can be used in various applications such as image retrieval, video surveillance, and virtual reality. 
However, the generated images may not always accurately represent the groups described in the prompt, especially when the generated images contain stereotypes. 


\begin{myDef}[\textbf{Stereotype}] The stereotype in a set of images is a widely held attribute associated with a specific group. If the probability density for a particular group exceeds a certain threshold in the images generated from the same prompts, we consider the stereotype associated with that group to be present. 
% It is formulated as follows: 
% \begin{equation}
%     \mathbf{s} = \mathbf{x}_1 \cap \mathbf{x}_2 \cap \dots \cap \mathbf{x}_i \cap \dots \cap \mathbf{x}_n,
% \end{equation}
% where
% \begin{equation}
% \begin{split}
%     \mathbf{x}_1 &= G(\mathbf{z}, \mathbf{\sigma}_1),\\
%     \mathbf{x}_2 &= G(\mathbf{z}, \mathbf{\sigma}_2),\\
%     &\dots\\
%     \mathbf{x}_i &= G(\mathbf{z}, \mathbf{\sigma}_i),\\
%     &\dots\\
%     \mathbf{x}_n &= G(\mathbf{z}, \mathbf{\sigma}_n).\\
% \end{split}
% \end{equation}

\end{myDef}

\begin{myDef}[\textbf{Stereotype Detection}]
Given a prompt $\mathbf{z}$, stereotype detection is the process of identifying whether the images generated by a Text-to-Image model $G$ contain stereotypes related to the group described in the input prompt. By denoting a stereotype extractor as $f$, we extract the stereotypes as follows:
\begin{equation}
    \hat{\mathbf{s}} = f(\mathbf{x})= f(G(\mathbf{z})),
\end{equation}
Then, the stereotype detection problem can be considered as a binary classification problem, by comparing the similarity between the stereotype $\hat{\mathbf{s}}$ extracted from generated images and the actual stereotypes $\mathbf{s}$: 
\begin{equation}
    \hat{y} = similarity(\hat{\mathbf{s}}, \mathbf{s}).
\end{equation}
\end{myDef}

==> sections/research_questions.tex <==
The objective of this study is to investigate the following research questions.

\textbf{Q1 (Text-to-Image models evaluation)}: \textit{Do widely-used Text-to-Image models generate stereotypical images?} This question examines the performance of widely-used Text-to-Image models to generate images based on textural prompts related to various demographic groups, such as gender, race, and religion.

\textbf{Q2 (Stereotype detectors evaluation)}: \textit{Could widely-studied object detectors accurately identify stereotypes in the images generated by the Text-to-Image models?} This question investigates the ability of widely-used stereotype detectors to classify stereotypical images related to various demographic groups.





% \subsection{Definition and Taxonomy}
% Bias in model generation may stem from biases inherent in the training data. ~\cite{} illustrates that a model's performance concerning fairness metrics can be significantly influenced by the approach taken to train the model on data representing underrepresented demographic groups. In the context of text-to-image model, biased prompts tend to overproduce images specifically related to a particular group, leading to the generation of stereotypes, such as "a thug" often producing images related to 'African'.

% For this issue, we design our bias dataset using a "(prompt, group)" format, which we refer to as the bias-group dataset. In this format, 'group' represents a demographic group in various statistical senses, such as Asians, Christians, etc. Furthermore, we categorize the target groups of bias into three dimensions: race and ethnicity, gender and sex, and religion. Each dimension encompasses various groups; for example, the “race and ethnicity” category includes classes such as African and Asian.

% By adopting this format and taxonomy, we aim to evaluate as comprehensively as possible the impact and degree of bias in current popular text-to-image models.
